Planning Shorter Paths in Graphs of Convex Sets by Undistorting Parametrized Configuration Spaces

Optimization based motion planning provides a useful modeling framework through various costs and constraints. Using Graph of Convex Sets (GCS) for trajectory optimization gives guarantees of feasibility and optimality by representing configuration space as the finite union of convex sets. Nonlinear parametrizations can be used to extend this technique to handle cases such as kinematic loops, but this distorts distances, such that solving with convex objectives will yield paths that are suboptimal in the original space. We present a method to extend GCS to nonconvex objectives, allowing us to "undistort" the optimization landscape while maintaining feasibility guarantees. We demonstrate our method's efficacy on three different robotic planning domains: a bimanual robot moving an object with both arms, the set of 3D rotations using Euler angles, and a rational parametrization of kinematics that enables certifying regions as collision free. Across the board, our method significantly improves path length and trajectory duration with only a minimal increase in runtime. Website: https://shrutigarg914.github.io/pgd-gcs-results/

==> figures/KDE_bimanual.tex <==
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/bimanual_path_length.png}
        \caption{The paths show on average 20.60\% shorter paths in $\mathbb{R}^{14}$  \tccomment{We'll probably have to remove these to save space. But we can still include them on a website for the paper. In that case, can we manually annotate the mean (draw a line and write the number)}}
        \label{fig:dist_comp}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/bimanual_traj_time.png}
        \caption{On average the trajectories are 31\% shorter after re-timing}
        \label{fig:trajt_comp}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/imbalance.png}
        \caption{The new trajectories are generally 0.2 points more in favour of the subordinate arm than the leading arm.}
        \label{fig:bal_comp}
    \end{subfigure}
    \caption{KDE plots for data collected from solving for 100 random paths generated by randomly sampling start and end points. Overall the improvement introduced by the post-processing step seems to be considerable. \tccomment{We should explicitly discuss somewhere why it gets worse (and mention it near this figure or where we explain it in the text)}}\label{fig:KDE Plots}
\end{figure}


==> tables/ciris_pgd.tex <==
\begin{table}[htbp]
    \centering
    \caption{Optimizing over the Nonconvex Cost Improves path length metric for the Three Benchmark Trajectories. \sgcomment{just for our reference- I don't think this table is worth space in the paper}
    }
    \label{tab:ciris_tmb}
    \begin{tabular}{|l|c|c|}
        \hline
        % \multicolumn{3}{|c|}{Path Lengths}\\
        % \hline
        & GCS & PGD \\
        \hline
        Top to Middle & 3.063 & 3.049 \\
        % \hline
        % Trajectory Time & 4.37 & 4.35 \\
        % \hline
        % \hline
        % \multicolumn{3}{|c|}{Top to Bottom}\\
        % \hline
        % & GCS & PGD \\
        \hline
        Top to Bottom & 3.89 & 3.83 \\
        % \hline
        % Trajectory Time & 5.96 & 6.09 \\
        \hline
        % \hline
        % \multicolumn{3}{|c|}{Middle to Bottom}\\
        % \hline
        % & GCS & PGD \\
        % \hline
        Middle to Bottom & 3.06 & 3.02 \\
        % \hline
        % Trajectory Time & 4.69 & 4.46 \\
        \hline

    \end{tabular}
\end{table}


==> tables/curvature.tex <==
\begin{table}[htbp]
    \centering
    \caption{Optimizing over the Nonconvex Cost Improves Metrics for the Three Benchmark Trajectories.
    \sgcomment{Add row for curvature??}
    }
    \label{tab:topmiddlebottom}
    \begin{tabular}{|l|c|c|}
        \hline
        \multicolumn{3}{|c|}{Top to Middle}\\
        \hline
        & GCS & PGD \\
        \hline
        R14 Path Length & 4.891 & 5.057 \\
        \hline
        Trajectory Time & 5.54 & 4.257 \\
        \hline
        \hline
        \multicolumn{3}{|c|}{Middle to Bottom}\\
        \hline
        & GCS & PGD \\
        \hline
        R14 Path Length & 3.531 & 3.647 \\
        \hline
        Trajectory Time &  5.168 & 3.58 \\
        \hline
        \hline
        \multicolumn{3}{|c|}{Top to Bottom}\\
        \hline
        & GCS & PGD \\
        \hline
        R14 Path Length & 6.821 & 6.928 \\
        \hline
        Trajectory Time &  7.59 & 5.68 \\
        \hline

    \end{tabular}
\end{table}


==> tables/woc_bench.tex <==
\begin{table}[htbp]
    \centering
    \caption{Optimizing over the Nonconvex Cost Improves Metrics for the Three Benchmark Trajectories. R14 path length and trajectory times decrease and imbalance gets approaches 0
    \sgcomment{Populate column for GCS+PGD+Curvature}
    \sgcomment{Add row for curvature??}
    }
    \label{tab:topmiddlebottom}
    \begin{tabular}{|l|c|c|}
        \hline
        \multicolumn{3}{|c|}{Top to Middle}\\
        \hline
        & GCS & GCS+PGD \\
        \hline
        R14 Path Length & 4.616 & 3.766 \\
        \hline
        Imalance & 0.26 & 0.14 \\
        \hline
        Trajectory Time & 4.172 & 3.469 \\
        \hline
        \hline
        \multicolumn{3}{|c|}{Middle to Bottom}\\
        \hline
        & GCS & PGD \\
        \hline
        R14 Path Length & 3.531 & 3.184 \\
        \hline
        Imalance & 0.18 & 0.098 \\
        \hline
        Trajectory Time & 3.77 & 3.16 \\
        \hline
        \hline
        \multicolumn{3}{|c|}{Bottom to Top}\\
        \hline
        & GCS & GCS+PGD \\
        \hline
        R14 Path Length & 6.376 & 5.191 \\
        \hline
        Imalance & 0.22 & 0.085 \\
        \hline
        Trajectory Time & 5.391 & 4.344 \\
        \hline

    \end{tabular}
\end{table}

